Fast solvers for the high-order FEM simplicial de Rham complex: Extended edition

We present new finite elements for solving the Riesz maps of the de Rham complex on triangular and tetrahedral meshes at high order. The finite elements discretize the same spaces as usual, but with different basis functions, so that the resulting matrices have desirable properties. These properties mean that we can solve the Riesz maps to a given accuracy in a $p$-robust number of iterations with $\mathcal{O}(p^6)$ flops in three dimensions, rather than the na\"ive $\mathcal{O}(p^9)$ flops. The degrees of freedom build upon an idea of Demkowicz et al., and consist of integral moments on an equilateral reference simplex with respect to a numerically computed polynomial basis that is orthogonal in two different inner products. As a result, the interior-interface and interior-interior couplings are provably weak, and we devise a preconditioning strategy by neglecting them. The combination of this approach with a space decomposition method on vertex and edge star patches allows us to efficiently solve the canonical Riesz maps at high order. We apply this to solving the Hodge Laplacians of the de Rham complex with novel augmented Lagrangian preconditioners.

==> figures/table_riesz_box.tex <==
\begin{table}[htbp]
	\centering
	\caption{PCG iteration counts to solve the $\Hgrad$ Riesz map, where $Y^0 = X^0_{\interface} \ (Y^0 = X^0)$. \label{tab:hgrad-unit-cube}}
	\csvreader[
	head to column names, head to column names prefix=MY,
	tabular=rcccc,
	table head=\toprule 
	& & \multicolumn{3}{c}{$\pafw{0}{Y^0}$} \\
	{$l$} & {$p$} & {$\alpha=10^3$} & {$\alpha=1$} & {$\alpha=10^{-3}$}\\
	\midrule,
	late after line=\ifthenelse{\equal{\MYdegree}{5}}{\\\midrule}{\\},
	filter ifthen=\equal{\MYdegree}{5} \or\equal{\MYdegree}{6} \or\equal{\MYdegree}{7},
	table foot=\bottomrule
	]{results/CG.3d.demkowicz.afw.combined.csv}{}
	{\MYlevel{} & \MYdegree{} & \MYFAiterations{} (\MYAiterations{})  & \MYFBiterations{} (\MYBiterations{}) & \MYFCiterations{} (\MYCiterations{})}
\end{table}

\begin{table}[htbp]
	\centering
	\footnotesize
	\caption{PCG iteration counts to solve the $\Hcurl$ Riesz map, where $Y^k = X^k_{\interface} \ (Y^k = X^k)$.\label{tab:hcurl-unit-cube}}
	\csvreader[
	head to column names, head to column names prefix=MY,
	tabular=r@{\hskip 0.75em}c@{\hskip 0.75em}c@{\hskip 0.75em}c@{\hskip 0.75em}c|,
	table head=\toprule 
	& & \multicolumn{3}{c|}{$\pafw{0}{Y^1}$} \\
	{$l$} & {$p$} & {$\alpha=10^3$} & {$\alpha=1$} & {$\alpha=10^{-3}$}\\
	\midrule,
	late after line=\ifthenelse{\equal{\MYdegree}{3}}{\\\midrule}{\\},
	filter ifthen=\equal{\MYdegree}{3} \or\equal{\MYdegree}{5} \or\equal{\MYdegree}{7},
	table foot=\bottomrule
	]{results/N1curl.3d.demkowicz.afw.combined.csv}{}
	{\MYlevel{} & \MYdegree{} & \MYFAiterations{} (\MYAiterations{})  & \MYFBiterations{} (\MYBiterations{}) & \MYFCiterations{} (\MYCiterations{})}
	%
	\hspace{-0.7em}
	%
	\csvreader[
	head to column names, head to column names prefix=MY,
	tabular=|c@{\hskip 0.75em}c@{\hskip 0.75em}c|,
	table head=\toprule
	\multicolumn{3}{c|}{$\ph{Y^0}{Y^1}$}\\ 
	{$\alpha=10^3$} & {$\alpha=1$} & {$\alpha=10^{-3}$}\\
	\midrule,
	late after line=\ifthenelse{\equal{\MYdegree}{3}}{\\\midrule}{\\},
	filter ifthen=\equal{\MYdegree}{3} \or\equal{\MYdegree}{5} \or\equal{\MYdegree}{7},
	table foot=\bottomrule
	]{results/N1curl.3d.demkowicz.hiptmair.combined.csv}{}
	{\MYFAiterations{} (\MYAiterations{})  & \MYFBiterations{} (\MYBiterations{}) & \MYFCiterations{} (\MYCiterations{})}
	\hspace{-0.7em}
	\csvreader[
	head to column names, head to column names prefix=MY,
	tabular=|c@{\hskip 0.75em}c@{\hskip 0.75em}c,
	table head=\toprule
	\multicolumn{3}{c}{$\ph{Y^0}{Y^{1,\rmone}}$}\\ 
	{$\alpha=10^3$} & {$\alpha=1$} & {$\alpha=10^{-3}$}\\
	\midrule,
	late after line=\ifthenelse{\equal{\MYdegree}{3}}{\\\midrule}{\\},
	filter ifthen=\equal{\MYdegree}{3} \or\equal{\MYdegree}{5} \or\equal{\MYdegree}{7},
	table foot=\bottomrule
	]{results/N1curl.3d.demkowicz.hiptmair-red.combined.csv}{}
	{\MYFAiterations{} (\MYAiterations{})  & \MYFBiterations{} (\MYBiterations{}) & \MYFCiterations{} (\MYCiterations{})}
\end{table}

\begin{table}[htbp]
	\centering
	\caption{PCG iteration counts to solve the $\Hdiv$ Riesz map, where $Y^k = X^k_{\interface} \ (Y^k = X^k)$.\label{tab:hdiv-unit-cube}}
	\csvreader[
	head to column names, head to column names prefix=MY,
	tabular=rlccc|,
	table head=\toprule 
	&  & \multicolumn{3}{c|}{$\pafw{0}{Y^2}$} \\
	{$l$} & {$p$} & {$\alpha=10^3$} & {$\alpha=1$} & {$\alpha=10^{-3}$}\\
	\midrule,
	late after line=\ifthenelse{\equal{\MYdegree}{3}}{\\\midrule}{\\},
	filter ifthen=\equal{\MYdegree}{3} \or\equal{\MYdegree}{5} \or\equal{\MYdegree}{7}
	]{results/N1div.3d.demkowicz.afw0.combined.csv}{}
	{\MYlevel{} & \MYdegree{} & \MYFAiterations{} (\MYAiterations{})  & \MYFBiterations{} (\MYBiterations{}) & \MYFCiterations{} (\MYCiterations{})}
	%
	\hspace{-0.7em}
	%
	\csvreader[
	head to column names, head to column names prefix=MY,
	tabular=|ccc,
	table head=\toprule 
	\multicolumn{3}{c}{$\pafw{1}{Y^2}$} \\
	{$\alpha=10^3$} & {$\alpha=1$} & {$\alpha=10^{-3}$}\\
	\midrule,
	late after line=\ifthenelse{\equal{\MYdegree}{3}}{\\\midrule}{\\},
	filter ifthen=\equal{\MYdegree}{3} \or\equal{\MYdegree}{5} \or\equal{\MYdegree}{7}
	]{results/N1div.3d.demkowicz.afw.combined.csv}{}
	{\MYFAiterations{} (\MYAiterations{})  & \MYFBiterations{} (\MYBiterations{}) & \MYFCiterations{} (\MYCiterations{})}
	
	% next row
	\csvreader[
	head to column names, head to column names prefix=MY,
	tabular=rlccc|,
	table head= \toprule
	&  & \multicolumn{3}{c|}{$\ph{Y^1}{Y^2}$} \\
	{$l$} & {$p$} & {$\alpha=10^3$} & {$\alpha=1$} & {$\alpha=10^{-3}$}\\
	\midrule,
	late after line=\ifthenelse{\equal{\MYdegree}{3}}{\\\midrule}{\\},
	filter ifthen=\equal{\MYdegree}{3} \or\equal{\MYdegree}{5} \or\equal{\MYdegree}{7},
	table foot=\bottomrule
	]{results/N1div.3d.demkowicz.hiptmair.combined.csv}{}
	{\MYlevel{} & \MYdegree{} & \MYFAiterations{} (\MYAiterations{})  & \MYFBiterations{} (\MYBiterations{}) & \MYFCiterations{} (\MYCiterations{})}
	%
	\hspace{-0.7em}
	%
	\csvreader[
	head to column names, head to column names prefix=MY,
	tabular=|ccc,
	table head= \toprule
	\multicolumn{3}{c}{$\ph{Y^{1,\rmone}}{Y^{2,\rmone}}$} \\
	{$\alpha=10^3$} & {$\alpha=1$} & {$\alpha=10^{-3}$}\\
	\midrule,
	late after line=\ifthenelse{\equal{\MYdegree}{3}}{\\\midrule}{\\},
	filter ifthen=\equal{\MYdegree}{3} \or\equal{\MYdegree}{5} \or\equal{\MYdegree}{7},
	table foot=\bottomrule
	]{results/N1div.3d.demkowicz.hiptmair-red.combined.csv}{}
	{\MYFAiterations{} (\MYAiterations{})  & \MYFBiterations{} (\MYBiterations{}) & \MYFCiterations{} (\MYCiterations{})}
\end{table}






